SoftSnap: Rapid Prototyping of Untethered Soft Robots Using Snap-Together Modules

Soft robots offer adaptability and safe interaction with complex environments. Rapid prototyping kits that allow soft robots to be assembled easily will allow different geometries to be explored quickly to suit different environments or to mimic the motion of biological organisms. We introduce SoftSnap modules: snap-together components that enable the rapid assembly of a class of untethered soft robots. Each SoftSnap module includes embedded computation, motor-driven string actuation, and a flexible thermoplastic polyurethane (TPU) printed structure capable of deforming into various shapes based on the string configuration. These modules can be easily connected with other SoftSnap modules or customizable connectors. We demonstrate the versatility of the SoftSnap system through four configurations: a starfish-like robot, a brittle star robot, a snake robot, a 3D gripper, and a ring-shaped robot. These configurations highlight the ease of assembly, adaptability, and functional diversity of the SoftSnap modules. The SoftSnap modular system offers a scalable, snap-together approach to simplifying soft robot prototyping, making it easier for researchers to explore untethered soft robotic systems rapidly.

==> sections/introduction-devin.tex <==
\section*{Introduction}
\label{sec:introduction}

\begin{figure}[b]
    \centering
    \includegraphics[width=\linewidth]{images/Overview.png}
    \caption{\textbf{Overview of the prototyping process.} The first row demonstrates that combining $n$ SoftSnap modules with a customized connector can construct a soft robot. The second row illustrates a gripper robot made from four SoftSnap modules arranged in a square and connected in the center. The third row depicts a brittle star-like robot created with five SoftSnap modules in a pentagonal configuration, also connected centrally. }
    \label{fig:overview}
\end{figure}

% soft robot 
% Lego idea 
%Systems like Legos facilitate the rapid prototyping of static structures and articulated rigid-body robots. This enables easy component reuse and rapid testing of different ideas about mechanical design, control, and applications. 

Soft robots are adaptable and compliant, enabling safe manipulation of delicate objects and navigation through challenging terrain, with applications in medical devices and search and rescue operations~\cite{lee2017soft, rus2015design, dong2022recent, zhao1}. 
Integrating controllers, batteries, actuators, and sensors into untethered, compliant systems poses a challenge due to the complexity of the assembly process~\cite{lee2017soft}. 

This paper introduces a technique and components for quickly prototyping soft robots, in the way that Legos and similar kits have enabled rapid prototyping of articulated rigid-body robots. The system is primarily intended for scientists with a range of backgrounds interested in exploring robotic analogs of biological organisms, or soft robot geometries suitable for manipulation or locomotion tasks. The system enables easy component reuse and rapid testing of different ideas about mechanical design, control, and applications. In addition to hardware and control software, we also describe a software simulator intended to be useful for a human designer; the simulator computes predicted shapes of the cable-driven modules as the cable length changes.

We demonstrate the versatility of the snap-together soft modular system through four distinct example assemblies: a gripper, a starfish robot, a snake robot, and a ring-shaped robot. 

Selection of the actuation method informs the design of a rapid-prototyping kit. Current actuation technologies for soft robots include pneumatic, cable-driven, electrically-responsive, magnetically-responsive, and thermal-responsive systems (e.g., shape memory alloys)~\cite{2024_Lee,zebing,rus2015design,schmitt2018soft,zhao1}. Pneumatic actuation, for example, is widely used for its simplicity and smooth, fluid-like motion~\cite{9785890}, but typically requires external pumps and tubing, limiting its practicality for untethered applications~\cite{9785890}. 
%Addressing these issues raises a key scientific question: how can we design systems that rapidly prototype untethered, adaptable, compliant soft robots?

%Modular robot related work

Modular robots, which inspire our snap-together prototyping system, can adapt their physical structure to different tasks through reconfiguration~\cite{liang2023decoding, zhao1, zhao2,ModularSR,Yim2002ModularRobots,reconfig_review,4141032}. Most modular robots rely on rigid components~
\cite{liang2023decoding,reconfig_review,Yim2002ModularRobots}. 
%which limits their ability to safely interact with complex environments~
Recent research has begun integrating soft robotics principles into modular designs, aiming to develop reconfigurable soft robots that combine compliance and adaptability for diverse applications~\cite{ModularSR,zhao1,zhao2,Li2019JelloCubeAC}. However, these approaches often involve intricate manual pre-assembly of modules, making it difficulty to rapidly explore alternative geometries, or to scale up to very large numbers of modules~\cite{ModularSR,2024_Lee}. Simplifying the assembly process and designing soft modules that support rapid prototyping is therefore a promising area for research~\cite{schmitt2018soft}.



\begin{figure*}[htbp]
    \centering
    \includegraphics[width=\linewidth]{images/App.png}
    \caption{\textbf{Examples of the cable-driven SoftSnap modular system applied to bio-inspired robotic designs.} The image illustrates three robotic motions inspired by nature: starfish overturning, brittle star locomotion, and snake concertina locomotion. The right images show control signals for five modules, highlighted in blue, red, yellow, orange, and green. \textbf{(a)} The starfish-like robot replicates the turning-over behaviour observed in real starfish. At t = 0 s, the robot leans on a purple block shaped to resemble a starfish. Control signals, shown on the right, are applied to facilitate this movement. By t = 1.75 s, the robot achieves a similar posture to a real starfish, with its top leg raised. It continues to receive control signals until it falls due to gravity at t = 3.25 s. The robot vividly emulates starfish motion until t = 11.25 s, after which the control is switched off, and the robot relaxes, resembling a starfish resting on the seafloor.
    \textbf{(b)} The brittle star-inspired robot demonstrates locomotion through periodic movements with a cycle of 1 s. Initially, the robot lies flat with its legs extended. A large step control signal is applied for 0.5 s, causing the legs to contract rapidly, followed by a zero control signal for the remaining 0.5 s to release the actuation quickly. This stretch and shrink motion generates momentum, moving the robot in a top-left direction, observable at t = 4 s, 6 s, and 10 s, showing clear displacement from its starting position.
    \textbf{(c)} The snake-like robot performs concertina locomotion by sequentially deforming its modules. In this demonstration, similar to (B), the robot exhibits a periodic motion with a cycle of 1.1 s. The four subfigures on the left-hand side illustrate the complete motion cycle of a snake robot: it starts in a straight position, contracts its body, achieves full contraction, begins to unwind, and progressively returns to its initial straight state from head to tail. This is achieved by periodically alternating the step signals in different colors. For example, with the yellow signal, we activate a step signal to the motor from 0 to 0.4 s, turn off the control from 0.4 to 0.9 s, and then reactivate the step signal from 0.9 to 1.1 s. The picture on the left shows that at t=0 s, the robot is in its initial state; at t=1 s, it begins to contract; at t=2 s, it is fully contracted; and by t=3 s, it is midway through returning to its original state. }
    \label{fig:applications1}
\end{figure*}

\begin{figure*}[htbp]
    \centering
    \includegraphics[width=\linewidth]{images/App2.png}
    \caption{Demonstrations of the cable-driven modular system applied to manipulation tasks. \textbf{(a)} The gripper robot effectively grasps objects of different shapes, such as a ball and a cuboid. In \textbf{a(i)}, we illustrate the five stages of ball grasping: standby and caging, where the modules remain in their initial state; sending a shrinking signal to four modules, which then bend to grasp the ball; lifting and steadying the ball; and finally, sending a release signal to the modules to return them to their initial state, allowing the ball to drop due to gravity. In \textbf{a(ii)}, we demonstrate grasping with three body shapes: one cuboid and two irregular forms, all controlled by the same signal for the four modules. \textbf{(b)} A four-module ring configuration is used for caging-type object transport, showcasing the ability to transport a large ball. At t = 0 s, the ring cage is in its initial state. At t = 6 s, the ball is placed inside the cage. By t = 10 s, all modules receive a control signal to contract, securing the ball from all directions. At t = 25 s, two parallel modules are activated to impart linear momentum to the ball, initiating movement. This process is repeated until the target is reached at t = 53 s, at which point the ball is released at the target.}
    \label{fig:applications2}
\end{figure*}


% djb -- already said this
%This paper presents a rapid prototyping system for soft robots that allows a human designer to rapidly explore different geometries of a certain class of soft robots. 
%We detail the design and initial implementation of cable-driven, modular soft actuator units 
% We present a design and first implementation of cable-driven, modular soft actuator units 
%that can be snapped together to quickly prototype untethered soft robotic systems. 
There are two main components in the SoftSnap system: (1) actuatable modules that each integrate a battery, motor, Wi-Fi communication, and control system, and (2) connectors that snap the modules together. Connectors can be easily 3D-printed to meet specific application requirements and can be re-used once built. Figure~\ref{fig:overview} displays an overview of the system, and Figure~\ref{fig:applications1} shows some biologically-inspired example robots we constructed with the system. 

Each SoftSnap module incorporates a passive skeleton with holes through which the actuating cable is threaded. Using different holes leads to different {\em threading configurations}, each of which leads to a different deformation pattern for the module. Snapping modules together is trivially easy; the slowest steps of building a new design include threading modules and possibly printing custom connectors. Once modules and connects of sufficient variety have been constructed, they form a kit that allows very fast exploration of new soft robot structures.

The SoftSnap modules, in some ways, serve a similar purpose to direct-driven joints in a traditional robot arm: the modules have one degree of freedom actuated by changing the cable length. Higher-degree-of-freedom serial or parallel structures for manipulation or locomotion can be formed by connecting these modules in various topologies using the connectors.  

Our current platform is meant to enable human designers to imagine, duplicate, or explore soft robot geometries. One difficulty in the process is that human designers may not have good intuition about what shapes a module with a particular threading pattern might achieve during actuation. We, therefore, present a quasi-static simulator that minimizes potential energy to predict the shapes achieved for different string lengths for a particular threading of the module. 
% Since there are finitely many threadings for a particular spine length with discrete threading holes, the simulator can construct a finite gallery of actuator shapes from which a human designer can select a threading with desired properties; see Figure~{ref:fig}. For simplicity, we only consider threadings such that at most one hole per spine is used.
%This model provides users with a sense of how the deformation shape of the skeleton looks with a certain threading, enhancing their understanding of the possible configurations. Building on this, 
We also modified the simulator for use as a design tool. This tool allows users to input a desired curve, and then attempts to find the threading design that most closely matches the curve. 




% djb verbose!
%These configurations showcase how the snap-together modules can be easily reassembled to create a range of functional soft robots, enabling untethered operation and supporting rapid prototyping. In this paper, we detail the design, modeling, and experimental validation of these modular soft robots, highlighting their adaptability for diverse applications.




